One Ring to Rule Them All: Certifiably Robust Geometric Perception with Outliers

We propose the first general and practical framework to design certifiable algorithms for robust geometric perception in the presence of a large amount of outliers. We investigate the use of a truncated least squares (TLS) cost function, which is known to be robust to outliers, but leads to hard, nonconvex, and nonsmooth optimization problems. Our first contribution is to show that -for a broad class of geometric perception problems- TLS estimation can be reformulated as an optimization over the ring of polynomials and Lasserre's hierarchy of convex moment relaxations is empirically tight at the minimum relaxation order (i.e., certifiably obtains the global minimum of the nonconvex TLS problem). Our second contribution is to exploit the structural sparsity of the objective and constraint polynomials and leverage basis reduction to significantly reduce the size of the semidefinite program (SDP) resulting from the moment relaxation, without compromising its tightness. Our third contribution is to develop scalable dual optimality certifiers from the lens of sums-of-squares (SOS) relaxation, that can compute the suboptimality gap and possibly certify global optimality of any candidate solution (e.g., returned by fast heuristics such as RANSAC or graduated non-convexity). Our dual certifiers leverage Douglas-Rachford Splitting to solve a convex feasibility SDP. Numerical experiments across different perception problems, including single rotation averaging, shape alignment, 3D point cloud and mesh registration, and high-integrity satellite pose estimation, demonstrate the tightness of our relaxations, the correctness of the certification, and the scalability of the proposed dual certifiers to large problems, beyond the reach of current SDP solvers.

==> methodology.tex <==
%!TEX root = main.tex

\section{Methodology}
As seen from examples~\ref{ex:essentialMatrix}-\ref{ex:3Dregistration}, the residual functions are typically quadratic convex functions of $\vxx$,~\ie~$r^2(\vxx,\vm_i) = \vxx\tran \MQ_i \vxx + 2 \vc_i\tran \vxx + a_i$. In addition, we assume the non-convex set $\calX$ can be described by \emph{polynomial equality and inequality} constraints,~\ie~$\calX \doteq \{\vxx \in \Real{n}: h_j(\vxx)=0,j=1,\dots,m; g_k(\vxx) \geq 0,k=1,\dots,l\}$. In addition, using the fact that $\min(x,y) = \min_{\theta = \pm 1} \frac{1+\theta}{2} x + \frac{1-\theta}{2} y$, we can rewrite problem~\eqref{eq:generalTLS} as:
\bea
\vxx^\star, \vtheta^\star =  & \displaystyle \argmin_{\vxx, \vtheta} \frac{1+\theta_i}{2} \left( \vxx\tran \MQ_i \vxx + 2 \vc_i\tran \vxx + a_i \right) + \frac{1-\theta_i}{2} \barcsq, \label{eq:TLStheta_obj}\\
\subject & p_i(\vtheta) = \theta_i^2 - 1 = 0, i=1,\dots,N,\\
 & h_j(\vxx)=0,j=1,\dots,m, \\
 &  g_k(\vxx) \geq 0,k=1,\dots,l,
\eea
where we have introduced $\vtheta = [ \theta_1,\dots,\theta_N ]\tran \in \{ \pm 1 \}^N$ as a vector of \emph{binary variables} such that each $\theta_i$ determines if the $i$-th measurement is an inlier ($\theta_i = + 1$) or an outlier ($\theta_i = -1$). The formulation in~\eqref{eq:TLStheta_obj} clearly exposes the combinatorial nature of the TLS estimation.

\subsection{Sums of Squares Relaxations}
We will leverage Lasserre's hierarchy of \emph{Sums of Squares} (SOS) relaxations and \emph{Moment} relaxations\footnote{SOS relaxations and moment relaxations are primal and dual semidefinite programs.} to solve problem~\eqref{eq:TLStheta_obj}~\cite{lasserre10book-momentsOpt}. 

\subsection{Exploiting Sparsity}
The size of the semidefinite program (SDP) resulting from Lasserre's hierarchy at relaxation order $\rorder$ is $\nchoosek{n+N+\rorder}{\rorder}$, which grows quickly intractable for problems of medium sizes (\eg~$n=10$, $N=20$, $\rorder = 2$). We will show that the problem formulation~\eqref{eq:TLStheta_obj} actually admits a special sparsity pattern such that it can be decomposed into smaller SDPs with $N$ PSD constraints, each having a much smaller size $\nchoosek{n+1+\rorder}{\rorder}$. Exploitation of the sparsity pattern will enable efficient solution of large-scale problems.

\subsection{Approximation Bounds}
In cases when the relaxation is \emph{not tight}, we will derive approximation bounds that \emph{a posteriori} quantify the quality of the \emph{rounded} solution.


==> problem_statement.tex <==
%!TEX root = main.tex

\section{Problem Statement}
We study \emph{robust geometric perception} using the \emph{truncated least squares} (TLS) cost function:
\bea \label{eq:generalTLS}
\vxx^\star = \argmin_{\vxx \in \calX} \sum_{i=1}^N \min \left( r^2(\vxx,\vm_i), \barcsq \right),
\eea
where $\vxx \in \calX$ is the unknown geometric quantity to be estimated (\eg~3D rotations $\MR \in \SOthree$), $\vm_i \in \calM,i=1,\dots,N$ are the given \emph{visual} measurements (\eg~pixel coordinates and 3D points), $r^2(\vxx,\vm_i)$ is the \emph{least squares residual} function that quantifies how well the measurements $\vm_i$'s agree with the unknown geometric quantity $\vxx$ (\eg~reprojection error and Euclidean distance), $\barcsq$ is a chosen constant (default $\barcsq=1$) that determines the \emph{maximum} allowed residual for \emph{inliers}. The second ``$\min$'' inside the summand in problem~\eqref{eq:generalTLS} implements the ``truncation'' of the TLS cost function, which performs \emph{least squares} estimation on inlier measurements whose residuals are smaller than $\barcsq$, while discards \emph{outlier} measurements whose residuals are larger than $\barcsq$\footnote{When $r^2(\vxx,\vm_i) > \barcsq$, $\min\left( r^2(\vxx,\vm_i), \barcsq \right) = \barcsq$ and a constant has no effect on the optimization.}. Therefore, the TLS estimation~\eqref{eq:generalTLS} is insensitive to large amounts of outliers~\cite{Yang19rss-teaser,Yang19iccv-QUASAR}.

In particular, we focus on instances of problem~\eqref{eq:generalTLS} where the function $r^2(\vxx, \vm_i)$ is a (convex) quadratic function of the unknown $\vxx$. We give three examples of problem~\eqref{eq:generalTLS} in geometric perception. 

\begin{example}[Robust Point Cloud Registration]\label{ex:3Dregistration} 
Let $\vxx = (\MR,\vt)$, where $\MR \in \SOthree, \vt \in \Real{3}$ is an unknown 3D rigid transformation to be estimated. The measurements set is $\calM = \{ \vm_i = (\va_i, \vb_i),i=1,\dots,N\}$, where $\va_i \in \Real{3}$ is the $i$-th 3D point in point cloud $\calA$, and $\vb_i$ is the $i$-th 3D point in point cloud $\calB$. The residual function is the Euclidean distance $r^2(\vxx,\vm_i) = d^2(\MR \va_i + \vt, P_i)/\beta_i^2$ between the transformed 3D point $\MR \va_i + \vt$ and the 3D primitive $P_i$\footnote{As shown in~\cite{Briales17cvpr-registration}, $d^2(\MR \va_i + \vt, P_i)$ can be written in closed-form as a quadratic function of $\MR$ and $\vt$.}, where $\beta_i$ is a constant that depends on the noise level of the measurements. The robust 3D registration problem seeks to find the best rigid transformation given 3D-3D correspondences $\va_i \leftrightarrow P_i$ that are potentially corrupted by a large amount of outliers. 
\end{example}

\begin{example}[Robust Mesh Registration]\label{ex:meshRegistration}
\bea
\min_{\MR \in \SOthree, \vt 
\in \Real{3}} \displaystyle \sum_{i=1}^N \min \left( \frac{\| \vb_i - \MR\va_i-\vt \|^2_{\vn_M\vn_M\tran}}{\beta_{P_i}^2} + \frac{\| \vn_{P_i} - \MR \vn_{M_i} \|^2}{\beta_{N_i}^2} ,2\barcsq\right)
\eea
\end{example}

\begin{example}[Robust Shape Alignment]\label{ex:shapeAlignment} 
Let $\vxx = (s,\MR,\vt)$, where $s>0,\MR \in \SOthree,\vt \in \Real{2}$ are the unknown scale, rotation and translation to be estimated. The measurements set is $\calM = \{\vm_i = (\vz_i, \MZ_i),i=1,\dots,N \}$, where $\vz_i \in \Real{2}$ is the $i$-th 2D landmark detected in an image, and $\MZ_i \in \Real{3}$ is the $i$-th 3D landmark in a 3D model. The residual function is the reprojection error $r^2(\vxx, \vm_i) = \| \vz_i - s \MPi \MR\MZ_i - \vt\|^2 / \beta_i^2$, where $\MPi \in \Real{2\times 3}$ is the weak perspective camera model and $\beta_i$ is a constant that depends on the noise level of the measurements. The robust shape alignment problem seeks to estimate the absolute pose of the 3D model given 2D-3D correspondences $\vz_i \leftrightarrow \MZ_i$ that are potentially corrupted by a large amount of outliers.
\end{example}



Examples~\ref{ex:essentialMatrix}-\ref{ex:3Dregistration} cover the entire spectrum of robust geometric perception given \emph{2D-2D}, \emph{2D-3D} and \emph{3D-3D} correspondences, which are of paramount importance in robotics and computer vision. Although \emph{globally optimal} solvers exist for the \emph{outlier-free} versions of examples~\ref{ex:essentialMatrix}-\ref{ex:3Dregistration}~\cite{Briales18cvpr-global2view,Yang20cvpr-shapeStar,Yang20ral-GNC,Horn87josa,Briales17cvpr-registration}, solving the robust estimation problem~\eqref{eq:generalTLS} is in general NP-hard, due to both non-convexity of the feasible set $\calX$ and the combinatorial nature of the TLS objective function\footnote{In fact, even if the feasible set $\calX$ is convex, problem~\eqref{eq:generalTLS} is still NP-hard in general~\cite{Liu19JCGS-minSumTruncatedConvexFunctions}.}. 

In this paper, we are interested in using state-of-the-art \emph{convex relaxations} to design \emph{certifiably robust} solvers for problem~\eqref{eq:generalTLS}, applied to the problems in examples~\ref{ex:essentialMatrix}-\ref{ex:3Dregistration}.
